Detecting Standard Violation Errors in Smart Contracts

We present SOLAR, a new analysis tool for automatically detecting standard violation errors in Ethereum smart contracts.Given the Ethereum Virtual Machine (EVM) bytecode of a smart contract and a user specified constraint or invariant derived from a technical standard such as ERC-20,SOLAR symbolically executes the contract, explores all possible execution paths, and checks whether it is possible to initiate a sequence of malicious transactions to violate the specified constraint or invariant. Our experimental results highlight the effectiveness of SOLAR in finding new errors in smart con-tracts. Out of the evaluated 779 ERC-20 and 310 ERC-721smart contracts, SOLAR found 255 standard violation errors in 197 vulnerable contracts with only three false positives.237 out of the 255 errors are zero-day errors that are not re-ported before. Our results sound the alarm on the prevalence of standard violation errors in critical smart contracts that manipulate publicly traded digital assets

==> __latexindent_temp.tex <==
 @misc{kaul_2016, title={IBM Watson IoT and Its Integration with Blockchain}, url={https://www.tractica.com/automation-robotics/ibm-watson-iot-and-its-integration-with-blockchain/}, author={Kaul, Aditya}, year={2016}, month={Aug}} 

==> figures/callalgo.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{try}{try}{:}{}
\SetKwProg{catch}{catch}{:}{end}
\underline{function} $ExecuteTransaction(\Sigma, T):$\\
\Input{live states $\Sigma$, transaction $T$}
\Output{live states $\Sigma^{'}$ after executing transaction}
\Begin{
% $T\leftarrow \langle a_s,a_c,v,d\rangle$\;
$\Sigma^{'}\leftarrow\emptyset$\;
\For {$\langle\sigma,\Gamma\rangle\in\Sigma$} {
    $\sigma_b(a_s)\leftarrow \sigma_b(a_s)-v$\;
    $\sigma_b(a_c)\leftarrow \sigma_b(a_c)+v$\;
    $\mu\leftarrow InitializeMachineState()$\;
    $\langle\mu,\sigma,T\rangle\lll\rrr\langle\bullet,\sigma_0,T_0\rangle\cdot\langle\bullet,\sigma_1,T_1\rangle\cdot\dots\cdot\langle\bullet,\sigma_n,T_n\rangle$\;
    $\Sigma^{'}\leftarrow\Sigma^{'}\cdot\langle\sigma_0,\Gamma\cdot T_0\rangle\cdot\langle\sigma_1,\Gamma\cdot T_1\rangle\cdot\dots\cdot\langle\sigma_n,\Gamma\cdot T_n\rangle$\;
}
}



==> figures/mainalgo-backup.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{try}{try}{:}{}
\SetKwProg{catch}{catch}{:}{end}
\underline{function} $Main(B, S, f):$\\
\Input{contract bytecode $B$, predefined address pool $S$, user defiend policies $f$}
\Begin{
\try{}{\label{start}
\For {$a\in S$} {
$b[a]\leftarrow 1000000$\;
}
$s[0\mapsto SymInt(),\dots,2^{256}-1\mapsto SymInt())]$\;
$\Gamma\leftarrow ExtractTransactions(f)$\;
$\psi\leftarrow ExtractConstraints(f)$\;
$\Sigma\leftarrow \langle\langle s, b, \psi\rangle,\emptyset\rangle$\;
\For{$T\in\Gamma$} {
    $\Sigma\leftarrow ExecuteTransaction(\Sigma, T)$
}

$GenerateReport(\Sigma)$\;
}
\catch{$e\leftarrow NewAddress(address)$}
{
$S\leftarrow S\cup e_{value}$\;
\kwGoTo \ref{start}\;
}
}



==> figures/opsemantics1.tex <==
\small
\centering
\noindent
\begin{gather*}
    \langle pc, k,\bullet,\bullet\rangle\lll \texttt{push } n\rrr \langle pc+1,n\cdot k,\bullet,\bullet\rangle \quad
    \langle pc,n\cdot k,\bullet,\bullet\rangle\lll \texttt{pop}\rrr \langle pc+1, k,\bullet,\bullet \rangle \\
    \langle pc,n_1\cdot n_2\cdot k,\bullet,\bullet\rangle\lll \texttt{add}\rrr \langle pc+1,n_1+n_2\cdot k,\bullet,\bullet\rangle \quad
    \langle pc,n_1\cdot 0\cdot k,\bullet,\bullet\rangle\lll \texttt{jumpi}\rrr \langle pc+1,k,\bullet,\bullet\rangle \\
    \frac{n_2\neq 0}{\langle\langle pc,n_1\cdot n_2\cdot k\rangle,\bullet,\bullet\rangle\lll \texttt{jumpi}\rrr \langle n_1,k,\bullet,\bullet\rangle} \quad
\end{gather*}


==> files/__latexindent_temp.tex <==
\begin{figure}


\begin{center}
    \begin{tabular}{ |c|c|c| } 
     \hline
     cell1 & cell2 & cell3 \\ 
     cell4 & cell5 & cell6 \\ 
     cell7 & cell8 & cell9 \\ 
     \hline
    \end{tabular}
    \end{center}
